Rollercoasters with Plateaus

In this paper we investigate the problem of detecting, counting, and enumerating (generating) all maximum length plateau-$k$-rollercoasters appearing as a subsequence of some given word (sequence, string), while allowing for plateaus. We define a plateau-$k$-rollercoaster as a word consisting of an alternating sequence of (weakly) increasing and decreasing \emph{runs}, with each run containing at least $k$ \emph{distinct} elements, allowing the run to contain multiple copies of the same symbol consecutively. This differs from previous work, where runs within rollercoasters have been defined only as sequences of distinct values. Here, we are concerned with rollercoasters of \emph{maximum} length embedded in a given word $w$, that is, the longest rollercoasters that are a subsequence of $w$. We present algorithms allowing us to determine the longest plateau-$k$-roller\-coasters appearing as a subsequence in any given word $w$ of length $n$ over an alphabet of size $\sigma$ in $O(n \sigma k)$ time, to count the number of plateau-$k$-rollercoasters in $w$ of maximum length in $O(n \sigma k)$ time, and to output all of them with $O(n)$ delay after $O(n \sigma k)$ preprocessing. Furthermore, we present an algorithm to determine the longest common plateau-$k$-rollercoaster within a set of words in $O(N k \sigma)$ where $N$ is the product of all word lengths within the set.

==> results2.tex <==
In this section we present our results regarding detecting, counting, and enumerating the set of plateau-$k$-rollercoasters 
that appear as a subsequence within a given word $w\in\Sigma^{n}$ for some $n \in \mathbb{N}$. 
Thus, we are extending the classical rollercoaster problem - given a word $w\in\Sigma^{\ast}$, determine the 
longest subsequence of $w$ which is a rollercoaster - to the plateau-rollercoaster scenario. We start with our 
algorithm for determining the longest plateau-$k$-rollercoaster appearing as a subsequence of a given word $w \in \Sigma^n$. To do so, we introduce two set of tables. First, the set of tables $L_{\xi}^{k, h}(w)$ (\textbf{L}ongest plateau-$(k,h)_{\xi}$-rollercoaster), with $L_{\xi}^{k, h}(w)[i]$ denoting the length of the longest plateau-$(k,h)_{\xi}$-rollercoaster in $w[i]$ ending at position $i$, noting that this may be different from the length of the longest plateau-$(k,h)_{\xi}$-rollercoaster in $w[i]$. We abuse our notation by using $L_{\xi}^{k, k}(w)[i]$ to denote the length of any proper plate-$k$-rollercoaster ending with a $\xi$-run at $w[i]$. Secondly, we have the $n \times \sigma$ table $P$ where $P(w)[i,x]$ contains the index $i'$ such that $i' \in [i]$ where $w[i'] = x$ and, $\forall j \in [i' + 1, i]$, $w[j] \neq x$.

\begin{remark}
Notice that $P_w$ can be constructed in time $O(n\sigma)$ for a given $w\in\Sigma^n$.
\end{remark}

\begin{lemma}
    \label{lem:L_k_h_table}
    Given a word $w \in \Sigma^n$ and triple of indices $i, k, h \in [n]$, the value of $L_{\xi}^{k, h}(w)[i]$ can be determined in $O(\sigma)$ time from the values of $L_{\xi'}^{k, h'}(w)[j]$, $\forall \xi' \in \{\uparrow, \downarrow\}, h' \in [k], j \in [i - 1]$.
\end{lemma}

\begin{proof}
    Observe that the longest plateau-$(k,h)_{\xi}$-rollercoaster ending at $w[i]$ must contain, as a prefix, some plateau-$(k,h')_{\xi'}$-rollercoaster ending at $w[j]$ for some $j \in [i -1 ]$, $h' \in [k]$ and $\xi' \in \{\uparrow, \downarrow\}$. Further, $j = P(w)[i - 1, w[j]]$, as otherwise there exists a longer plateau-$(k,h')_{\xi'}$-rollercoaster ending at $P(w)[i - 1, w[j]]$. Let us first assume that $\xi = \uparrow$ and note that the arguments may be trivially modified for $\xi = \downarrow$. If $h \in [2, k - 1]$, then we are looking for the value $j$ such that $w[j] \leq w[i]$ and $\forall j' \in [i - 1]$ where $w[j'] \leq w[i]$, either $L_{\uparrow}^{k, h - 1}(w)[j'] < L_{\uparrow}^{k, h - 1}(w)[j]$, if $w[j] \neq w[i]$, or $L_{\uparrow}^{k, h - 1}(w)[j'] < \max{L_{\uparrow}^{k, h}(w)[j], L_{\uparrow}^{k, h - 1}(w)[j]}$ if $w[j] = w[i]$. Note that this can be found by checking, in $O(\sigma)$ time, each value of $j \in \{P(w)[i - 1, x] \mid x \in \Sigma\}$ sequentially and choosing the value maximising the either $L_{\uparrow}^{k, h - 1}(w)[j]$, if $w[j] < w[i]$ or $\max{L_{\uparrow}^{k, h}(w)[j], L_{\uparrow}^{k, h - 1}(w)[j]}$ if $w[j] = w[i]$. Otherwise, if $h = 1$, then as $w[i]$ is the first element of a $\xi$-run, it must also be the last element of a $\overline{\xi}$-run, or continuing a plateau of the last element of such a run. As such, we are instead looking for the index $j \in \{P(w)[x] \mid x \in \Sigma\}$ maximising either $\max{L_{\downarrow}^{k, k}(w)[j], L_{\downarrow}^{k, k - 1}(w)[j]}$, if $w[j] > w[i]$, or $\max{L_{\downarrow}^{k, k}(w)[j], L_{\downarrow}^{k, k - 1}(w)[j], L_{\uparrow}^{k, 1}(w)[j]}$ if $w[j] = w[i]$. Again, this can be determined in $O(\sigma)$ time by checking each value of $j \in \{P(w)[i - 1, x] \mid x \in \Sigma\}$ sequentially. Finally, if $h = k$, then $w[i]$ is either the $k^{th}$ symbol of a run containing $k - 1$ symbols, the continuation of a plateau of a run containing at least $k$ unique symbols, or an extension of a run containing at least $k$ unique symbols. Therefore, the problem becomes determining the value of $j \in \{P(w)[i - 1, x] \mid x \in \Sigma\}$ maximising $\max(L_{\uparrow}^{k, k - 1}(w)[j], L_{\uparrow}^{k, k}(w)[j])$, if $w[j] < w[i]$, or $L_{\uparrow}^{k, k}(w)[j]$ if $w[j] = w[i]$, the value of which may be determined in $O(\sigma)$ time in the same manner as before.
\end{proof}

\begin{corollary}
    \label{col:full_L_j_h_table}
    Given a word $w \in \Sigma^n$, the value of $L_{\xi}^{k, h}(w)[i]$ can be determined in $O(n \sigma k)$ time for every $\forall \xi \in \{\uparrow, \downarrow\}, h \in [k], i \in [n]$.
\end{corollary}

\begin{theorem}
    \label{thm:length_of_the_longest_roller_coaster}
    Given a word $w \in \Sigma^n$, we can determine the length of the longest plateau-$k$-rollercoaster in $O(n \sigma k)$ time.
\end{theorem}

\begin{proof}
    From Corollary \ref{col:full_L_j_h_table}, we can construct the table $L_{\xi}^{k, h}(w)$ in $O(n \sigma k)$ time. By definition, the longest rollercoaster is the value $\max_{i \in [n]} L_{\xi}^{k, k}(w)[i]$, which may be determined in $O(n)$ time from $L_{\xi}^{k, h}(w)$, giving the stated time complexity.
\end{proof}

We now consider the problems of counting and enumerating the set of maximum-length rollercoasters in $w$. We do so via the \emph{$k$-rollercoaster table}, $R(w)$ of the word. Informally, $R(w)$ can be thought of as an extension of $L_{\xi}^{k, h}(w)$, storing not only the longest plateau-$(k,h)_{\xi}$-rollercoasters ending at each position, but also the number of such rollercoasters.

\begin{definition}[Rollercoaster Table]
    \label{def:rollercoaster_table}
    Given a word $w\in\Sigma^n$, for some $n \in \N$, and $k\in\N$, the \emph{rollercoaster table} of $w$ and $k$ is the table $R(w,k)$ of size $n \times 
    2 \times k$, indexed by the triples $(i, \xi, h)$ where $i \in [n]$, $\xi \in \{\uparrow,
    \downarrow\}$, and $h \in [0, k - 1]$, where $R(w,k)[(i, \xi, h)]$ is the number of subsequences $s$ which are plateau-$(k,h)_{\xi}$-rollercoasters
    ending at position $i$ in $w$, i.e. $w[i]$ is the last symbol of $s$.
\end{definition}

% The rollercoaster table of $w$ provides the main tool behind our algorithmic results. Observe that, once $R(w,k)$ has been computed, the longest rollercoasters that is a subsequence of $w$ can be determined in $O(n^2)$ time by finding the largest $j$ such that $R(w,k)[(i, j, \xi, 0)] > 0$ for any $i \in [n]$ and $\xi \in \{ \uparrow, \downarrow\}$.
We now outline our approach for computing $R(w,k)$, providing pseudocode for this algorithm in Algorithm \ref{alg:computing_R_w} and a proof of correctness in Theorem \ref{thm:computing_R_w}, using the table $L_{\xi}^{k, h}(w)$ as a basis.

% \begin{algorithm}
%    
%     \label{alg:computing_R_w}
%     \begin{algorithmic}
%         \Procedure{ComputeR}{word $w \in \Sigma^n$, $k \in \mathbb{N}$}
%             \State $R \gets $ empty table of size $n \times n \times 2 \times k$ \% \emph{we assume that every position starts at 0.}
%             \For{$i \in [n]$} \% \emph{Initially we populate the positions $R[i, 1, \xi, 1]$ as 1, for every $i \in [n], \xi \in \{\uparrow, \downarrow\}$}
%                 \State $R[i, 1, \uparrow, 1] \gets 1$ \% \emph{Representing the rollercoaster starting with an increasing run at position $i$.}
%                 \State $R[i, 1, \downarrow, 1] \gets 1$ \% \emph{Representing the rollercoaster starting with a decreasing run at position $i$.}
%             \EndFor
%             \For{$i, j \in [2, n], r \in [0, k - 1]$} \% \emph{Note that there exists no partial rollercoaster of length greater than 1 ending at position $1$, thus we can ignore it.}
%                 \For{$i' \in [i - 1]$}
%                     \If{$r = 0$}
%                         \If{$w[i] < w[i']$}
%                             \State $R[i, j, \uparrow, r] \gets R[i, j, \uparrow, r] + R[i', j - 1, \uparrow, 0] + R[i', j - 1, \downarrow, k - 1]$ \% \emph{Increases the value of $R[i, j, \xi, r]$ by the number of runs ending at $w[i']$ that has either just finished a decreasing run, and not started an increasing run, $R[i', j - 1, \xi, 0]$, or is one symbol away from completing a decreasing run, $R[i', j - 1, \downarrow, k - 1]$. Note that if $w[i] > w[i']$ then any run where $w[i]$ follows $w[i']$ can not be decreasing.}
%                         \ElsIf{$w[i] = w[i']$} \% \emph{If we are on a plateau we can only increase runs that are already finished.}
%                             \State $R[i, j, \uparrow, r] \gets R[i, j, \uparrow, r] + R[i', j - 1, \uparrow, 0]$
%                             \State $R[i, j, \downarrow, r] \gets R[i, j, \downarrow, r] + R[i', j - 1, \downarrow, 0]$
%                         \Else \% $w[i] > w[i']$
%                             \State $R[i, j, \downarrow, r] \gets R[i, j, \downarrow, r] + R[i', j - 1, \downarrow, 0] + R[i', j - 1, \uparrow, k - 1]$ \% \emph{Follows the same logic as above.}
%                         \EndIf
%                     \Else
%                         \If{$w[i] < w[i']$}
%                             \State $R[i, j, \downarrow, r] \gets R[i, j, \downarrow, r] + R[i', j, \downarrow, r - 1]$ \% \emph{Increases the value of $R[i, j, \downarrow, r]$ by the number of $r - 1$ partial rollercoasters ending at $w[i']$ of length $j - 1$, where $w[i] \leq w[i']$}
%                         \ElsIf{$w[i] = w[i']$} \% \emph{If we are on a plateau we can only increase runs that are of the same length.}
%                             \State $R[i, j, \downarrow, r] \gets R[i, j, \downarrow, r] + R[i', j, \downarrow, r]$
%                             \State $R[i, j, \uparrow, r] \gets R[i, j, \uparrow, r] + R[i', j, \downarrow, r]$
%                         \Else \% $w[i] \geq w[i']$
%                             \State $R[i, j, \uparrow, r] \gets R[i, j, \uparrow, r] + R[i, j, \uparrow, r - 1]$ \% \emph{Follows the same logic as above.}
%                         \EndIf
%                     \EndIf
%                 \EndFor
%             \EndFor
%             \State \Return{$R$}
%         \EndProcedure
%     \end{algorithmic} \caption{Our primary algorithmic tool for computing the rollercoaster table of a given word}
% \end{algorithm}


%    \begin{algorithm}\label{alg:computing_R_w}
%    \textbf{Input:} $w \in \Sigma^n$, $k \in \mathbb{N}$\\
%    \textbf{Output:} rollercoaster table $R$ for $w$ and $k$
    
% \begin{lstlisting}[mathescape=true]
% ComputeR($w \in \Sigma^n$, $k \in \mathbb{N}$)
%   // assume every position starts at 0
%   $R$ = empty table of size $n \times n \times 2 \times k$ 
%     
%   // Initialisation of $R[i,1,\xi,1]$ for increasing and decreasing starting runs
%   for $i\in[n]$
%     $R[i, 1, \uparrow, 1] = 1$ 
%     $R[i, 1, \downarrow, 1] = 1$ 
%         
%   // Computation of partial rollercoasters, starting by $2$, since no partial rollercoaster starts in $1$.
%   for $i, j \in [2, n], r \in [0, k - 1]$ 
%     for $i' \in [i - 1]$
%       if $r = 0$
%         if $w[i] < w[i']$
%         // Increases the value of $R[i, j, \xi, r]$ by the number of runs ending at $w[i']$ that has either just finished a decreasing run, and not started an increasing run, $R[i', j - 1, \xi, 0]$, or is one symbol away from completing a decreasing run, $R[i', j - 1, \downarrow, k - 1]$. Note that if $w[i] > w[i']$ then any run where $w[i]$ follows $w[i']$ can not be decreasing.  
%           $R[i, j, \uparrow, r] = R[i, j, \uparrow, r] + R[i', j - 1, \uparrow, 0] + R[i', j - 1, \downarrow, k - 1]$ 
%         else if $w[i] = w[i']$ 
%         // if we are on a plateau we can only increase runs that are already finished.
%           $R[i, j, \uparrow, r] = R[i, j, \uparrow, r] + R[i', j - 1, \uparrow, 0]$
%           $R[i, j, \downarrow, r] = R[i, j, \downarrow, r] + R[i', j - 1, \downarrow, 0]$
%         else
%           // as above
%           $R[i, j, \downarrow, r] = R[i, j, \downarrow, r] + R[i', j - 1, \downarrow, 0] + R[i', j - 1, \uparrow, k - 1]$
%       else
%         if $w[i] < w[i']$
%         // Increases the value of $R[i, j, \downarrow, r]$ by the number of $r - 1$ partial rollercoasters ending at $w[i']$ of length $j - 1$, where $w[i] \leq w[i']$
%           $R[i, j, \downarrow, r] = R[i, j, \downarrow, r] + R[i', j, \downarrow, r - 1]$ 
%         else if $w[i] = w[i']$ 
%         // if we are on a plateau we can only increase runs that are of the same length.
%           $R[i, j, \downarrow, r] = R[i, j, \downarrow, r] + R[i', j, \downarrow, r]$
%           $R[i, j, \uparrow, r] 0 R[i, j, \uparrow, r] + R[i', j, \downarrow, r]$
%         else 
%           $R[i, j, \uparrow, r] = R[i, j, \uparrow, r] + R[i, j, \uparrow, r - 1]$ 
%   return $R$          
% \end{lstlisting} 
% \caption{ComputeR}
% \end{algorithm}

\begin{algorithm}
\textbf{Input:} $w \in \Sigma^n$, $k \in \mathbb{N}$\\
\textbf{Output:} rollercoaster table $R$ for $w$ and $k$
\begin{lstlisting}[mathescape=true]
// assume every position starts at 0
$R$ = empty table of size $n \times 2 \times k$
Initialise $L_{\xi}^{k, h}(w)$, $\forall \xi \in \{\uparrow, \downarrow\}, h \in [k]$
Compute $P(w)$
// Initialisation of $R[i,\xi,1]$ for increasing and decreasing starting runs
for $i\in[n]$
  $R[i, \uparrow, 1] = 1$ 
  $R[i, \downarrow, 1] = 1$ 
// Computation of partial rollercoasters, starting by $2$, since no partial rollercoaster starts in $1$.
for $i \in [2, n], h \in [k]$ 
  for $i' \in \{P(w)[i - 1, x] \mid x \in \Sigma\}$
    if $h = 1$
      if $w[i] < w[i']$ and $L_{\uparrow}^{k, 1}(w)[i] = L_{\downarrow}^{k, k} + 1$
      // Increases the value of $R[i, \xi, 1]$ by the number of runs ending at $w[i']$ that have just finished a decreasing run, and not been marked as starting an increasing run, $R[i', \xi, k]$ Note that if $w[i] > w[i']$ then any run where $w[i]$ follows $w[i']$ can not be decreasing and thus must be the second element of some increasing run.
        $R[i, \uparrow, 1] = R[i, \uparrow, 1] + R[i', \downarrow, k]$
      if $w[i] < w[i']$ and $L_{\uparrow}^{k, 1}(w)[i] = L_{\downarrow}^{k, k - 1} + 1$
        // Increases the value of $R[i, \xi, 1]$ by the number of runs ending at $w[i']$ that are one element away from finishing a decreasing run, $R[i', \downarrow, k - 1]$. Note both this and the above case may be applied
        $R[i, \uparrow, 1] = R[i, \uparrow, 1] + R[i', \downarrow, k - 1]$ 
      // if we are on a plateau we can only increase runs that are already finished.
      if $w[i] = w[j]$ and  $L_{\uparrow}^{k, 1}(w)[i] = L_{\uparrow}^{k, 1}[i'] + 1$
        $R[i, \uparrow, 1] = R[i, j, \uparrow, 1] + R[i', \uparrow, 1]$
      if $w[i] = w[j]$ and  $L_{\downarrow}^{k, 1}(w)[i] = L_{\downarrow}^{k, 1}[i'] + 1$
        $R[i, \downarrow, 1] = R[i, \downarrow, r] + R[i', \downarrow, 1]$
      if $w[i] > w[i']$ and $L_{\downarrow}^{k, 1}(w)[i] = L_{\uparrow}^{k, k}[i'] + 1$
        // as above
        $R[i, \downarrow, 1] = R[i, \downarrow, 1] + R[i', \uparrow, k]$
      if $w[i] > w[i']$ and $L_{\downarrow}^{k, h}(w)[i] = L_{\uparrow}^{k, k - 1}[i'] + 1$
        // as above
        $R[i, \downarrow, r] = R[i, \downarrow, 1] + R[i', \uparrow, k - 1]$
    else
      if $w[i] < w[i']$ and $L_{\downarrow}^{k, h}(w)[i] = L_{\downarrow}^{k, h - 1}[i'] + 1$
      // Increases the value of $R[i, \downarrow, r]$ by the number of $h - 1$ partial rollercoasters ending at $w[i']$
        $R[i, \downarrow, h] = R[i, \downarrow, h] +  R[i', \downarrow, h - 1]$
      if $w[i] < w[i'], h = k$ and $L_{\downarrow}^{k, h}(w)[i] = L_{\downarrow}^{k, k}[i'] + 1$
      // Increases the value of $R[i, \downarrow, h] + R[i, \downarrow, h]$ if $h = k$ and $w[i]$ can still follow $w[i']$ in a rollercoaster of maximum length (note that the above case still applies)
        $R[i, \downarrow, h] = R[i, \downarrow, h] +  R[i', \downarrow, h]$
      // if we are on a plateau we can only increase runs that are of the same length
      if $w[i] = w[i']$ and $L_{\downarrow}^{k, h}(w)[i] = L_{\downarrow}^{k, h}[i'] + 1$
        $R[i, \downarrow, h] = R[i, \downarrow, h] + R[i',\downarrow, h]$
      if $w[i] = w[i']$ and $L_{\uparrow}^{k, h}(w)[i] = L_{\uparrow}^{k, h}[i'] + 1$
        $R[i, \uparrow, h] = R[i, \uparrow, r] + R[i', \downarrow, j]$
      if $w[i] > w[i']$ and $L_{\uparrow}^{k, h}(w)[i] = L_{\uparrow}^{k, h - 1}[i'] + 1$
        $R[i, \uparrow, h] = R[i, \uparrow, h] +  R[i', \uparrow, h - 1]$
      if $w[i] > w[i'], h = k$ and $L_{\uparrow}^{k, h}(w)[i] = L_{\uparrow}^{k, k}[i'] + 1$
      // Increases the value of $R[i, \downarrow, h] + R[i, \downarrow, h]$ if $h = k$ and $w[i]$ can still follow $w[i']$ in a rollercoaster of maximum length (note that the above case still applies)
        $R[i, \uparrow, h] = R[i, \uparrow, h] +  R[i', \uparrow, h]$
return $R$          
\end{lstlisting} 
\caption{ComputeR}\label{alg:computing_R_w}
\end{algorithm}

% TODO, Also make sure that we are correct with the way that we are handling $j = 1/2$ vs 0, since the end of an increasing run is also the start of a decreasing run & vice/versa. Maybe just need to get rid of $j = 0$?

\begin{theorem}
    \label{thm:computing_R_w}
    Algorithm \ref{alg:computing_R_w} returns the rollercoaster table for a given input word $w \in \Sigma^{n}$ and an integer $k$ as defined in Definition \ref{def:rollercoaster_table} in $O(n \sigma k)$ time.
\end{theorem}

\begin{proof}
    Observe that Algorithm \ref{alg:computing_R_w} computes $R(w,k)$ in a dynamic manner. As a base case, note the $R(w,k)[i, \xi, 1]$ is equal to $1$ for every $i \in [n], \xi \in \{\uparrow, \downarrow\}$, corresponding to the PP$1$R associated to position $i$, which may be either an increasing or decreasing run. In general, the value of $R(w,k)[i, \xi, h]$ can be computed by one of four summations, depending on the values of $\xi$ and $h$.

    If $h = 1$ and $\xi = \uparrow$, for $R(w,k)[i, \uparrow, 0]$ we have to count the number of subsequences that are $\downarrow$-PP$k$R of length $L_{\uparrow}^{k, 1}(w)[i]$ ending in $w[i]$. This equals the number of subsequences that are
    $\downarrow$-$(k-1)$PP$(L_{\uparrow}^{k, h}(w)[i] - 1)$R ending in any $i' \in \{P(w)[i - 1, x \mid x < w[i]]\}$ plus the number of subsequences that are $\uparrow$-$k$PP$(j-1)$R ending at $P(w)[i - 1, w[i]]$. Thus, we get with
    $I_{\diamond}= \{i' \in [i - 1] \mid  w[i'] \diamond w[i]\}$ for $\diamond\in\{<,>,\leq,\geq,=\}$

    $$
        R(w, k)[i, \uparrow, 1] = \sum_{i' \in \{P(w)[i - 1, x \mid x \in [w[i] - 1]\}} \begin{cases}
            R[i', \downarrow, k] & L_{\uparrow}^{k, 1}(w)[i] = L_{\downarrow}^{k, k}(w)[i'] + 1 \neq L_{\downarrow}^{k, k - 1}(w)[i'] + 1\\
            R[i', \downarrow, k- 1] & L_{\uparrow}^{k, 1}(w)[i] = L_{\downarrow}^{k, k - 1}(w)[i'] + 1 \neq L_{\downarrow}^{k, k}(w)[i']\\
            R[i', \downarrow, k] + R[i', \downarrow, k- 1] & L_{\uparrow}^{k, 1}(w)[i] = L_{\downarrow}^{k, k}(w)[i'] + 1 = L_{\downarrow}^{k, k - 1}(w)[i']\\
            0 & \text{\emph{otherwise}}
        \end{cases} + \begin{cases}
            R[P(w)[i - 1, w[i]], \downarrow, k] & L_{\uparrow}^{k, 1}(w)[i] = L_{\downarrow}^{k, k}(w)[[P(w)[i - 1, w[i]], \downarrow, k]] + 1 \neq L_{\downarrow}^{k, 1}(w)[[P(w)[i - 1, w[i]], \downarrow, k]] + 1\\
            R[[P(w)[i - 1, w[i]], \downarrow, k], \uparrow, 1] & L_{\uparrow}^{k, 1}(w)[i] = L_{\downarrow}^{k, 1}(w)[i'] + 1 \neq L_{\downarrow}^{k, k}(w)[[P(w)[i - 1, w[i]], \downarrow, k]]\\
            R[[P(w)[i - 1, w[i]], \downarrow, k], \downarrow, k] + R[[P(w)[i - 1, w[i]], \downarrow, k], \uparrow, 1] & L_{\uparrow}^{k, 1}(w)[i] = L_{\downarrow}^{k, k}(w)[[P(w)[i - 1, w[i]], \downarrow, k]] + 1 = L_{\downarrow}^{k, 1}(w)[[P(w)[i - 1, w[i]], \downarrow, k]]\\
            0 & \text{\emph{otherwise}}
        \end{cases}
    $$
    By an analogous argument we get that 
    $$
        R(w, k)[i, \uparrow, 1] = \sum_{i' \in \{P[i - 1, x] \mid x \in [w[i] + 1, \sigma] \}} \begin{cases}
            R[i', \uparrow, k] & L_{\downarrow}^{k, 1}(w)[i] = L_{\uparrow}^{k, k}(w)[i'] + 1 \neq L_{\uparrow}^{k, k - 1}(w)[i'] + 1\\
            R[i', \uparrow, k- 1] & L_{\downarrow}^{k, 1}(w)[i] = L_{\uparrow}^{k, k - 1}(w)[i'] + 1 \neq L_{\uparrow}^{k, k}(w)[i']\\
            R[i', \uparrow, k] + R[i', \downarrow, k- 1] & L_{\downarrow}^{k, 1}(w)[i] = L_{\uparrow}^{k, k}(w)[i'] + 1 = L_{\uparrow}^{k, k - 1}(w)[i']\\
            0 & \text{\emph{otherwise}}
        \end{cases} + \begin{cases} 
            R[P(w)[i - 1, w[i]], \uparrow, k] & L_{\downarrow}^{k, 1}(w)[i] = L_{\uparrow}^{k, k}(w)[P(w)[i - 1, w[i]]] + 1 \neq L_{\uparrow}^{k, 1}(w)[P(w)[i - 1, w[i]]] + 1\\
            R[P(w)[i - 1, w[i]], \downarrow, 1] & L_{\downarrow}^{k, 1}(w)[i] = L_{\uparrow}^{k, 1}(w)[P(w)[i - 1, w[i]]] + 1 \neq L_{\uparrow}^{k, k}(w)[P(w)[i - 1, w[i]]]\\
            R[P(w)[i - 1, w[i]], \uparrow, k] + R[P(w)[i - 1, w[i]], \downarrow, 1] & L_{\downarrow}^{k, 1}(w)[i] = L_{\uparrow}^{k, k}(w)[P(w)[i - 1, w[i]]] + 1 = L_{\uparrow}^{k, k - 1}(w)[P(w)[i - 1, w[i]]]\\
            0 & \text{\emph{otherwise}}
        \end{cases}.
    $$
    If $h > 1$ and $\xi = \uparrow$ we have that any subsequence which is a $h$PP$L_{\uparrow}^{k, 1}(w)[i]$R ending at $w[i]$ has to be a subsequence which is either an $(h - 1)$PP$(L_{\uparrow}^{k, 1}(w)[i] - 1)$R ending at some position $i' \in \{P(w)[i - 1, x] \mid x \in [w[i] - 1] \}$, or an $h$PP$(L_{\uparrow}^{k, 1}(w)[i]-1)$R  ending at $P(w)[i - 1, w[i]]$. This gives us, with the above notation
    \[
    R(w,k)[i, \uparrow, h] =
    \sum_{i' \in \{P(w)[i - 1, x] \mid x \in [w[i] - 1]\}} \begin{cases}
        R[i', \uparrow, h - 1] &  L_{\uparrow}^{k, h}(w)[i] = L_{\uparrow}^{k, h - 1}(w)[i'] + 1 \text{ and } h \neq k\\
        R[i', \uparrow, h - 1] &  L_{\uparrow}^{k, h}(w)[i] = L_{\uparrow}^{k, h - 1}(w)[i'] + 1, h = k \text{ and } L_{\uparrow}^{k, h}(w)[i] = \neq L_{\uparrow}^{k, k}(w)[i'] + 1\\
        R[i', \uparrow, h] &  L_{\uparrow}^{k, h}(w)[i] \neq L_{\uparrow}^{k, h - 1}(w)[i'] + 1, h = k \text{ and } L_{\uparrow}^{k, h}(w)[i] = L_{\uparrow}^{k, k}(w)[i'] + 1\\
        R[i', \uparrow, h - 1] + R[i', \uparrow, h] &  L_{\uparrow}^{k, h}(w)[i] \neq L_{\uparrow}^{k, h - 1}(w)[i'] + 1, h = k \text{ and } L_{\uparrow}^{k, h}(w)[i] = L_{\uparrow}^{k, k}(w)[i'] + 1\\
        0 & \text{\emph{otherwise}}
    \end{cases} + 
        R[[P(w)[i - 1, w[i]], \uparrow, h] &  L_{\uparrow}^{k, h}(w)[i] = L_{\uparrow}^{k, h}(w)[[P(w)[i - 1, w[i]]] + 1\\
        0 & \text{\emph{otherwise}}
    \]
    Analogously, we get 
    \[
    R(w,k)[i, \downarrow, h] =
    \sum_{i' \in \{P(w)[i - 1, x] \mid x \in [w[i] + 1, \sigma] \}} \begin{cases}
        R[i', \downarrow, h - 1] &  L_{\downarrow}^{k, h}(w)[i] = L_{\downarrow}^{k, h - 1}(w)[i'] + 1 \text{ and } h \neq k\\
        R[i', \downarrow, h - 1] &  L_{\downarrow}^{k, h}(w)[i] = L_{\downarrow}^{k, h - 1}(w)[i'] + 1, h = k \text{ and } L_{\downarrow}^{k, h}(w)[i] = \neq L_{\downarrow}^{k, k}(w)[i'] + 1\\
        R[i', \downarrow, h] &  L_{\downarrow}^{k, h}(w)[i] \neq L_{\downarrow}^{k, h - 1}(w)[i'] + 1, h = k \text{ and } L_{\downarrow}^{k, h}(w)[i] = L_{\downarrow}^{k, k}(w)[i'] + 1\\
        R[i', \downarrow, h - 1] + R[i', \uparrow, h] &  L_{\downarrow}^{k, h}(w)[i] \neq L_{\downarrow}^{k, h - 1}(w)[i'] + 1, h = k \text{ and } L_{\downarrow}^{k, h}(w)[i] = L_{\downarrow}^{k, k}(w)[i'] + 1\\
        0 & \text{\emph{otherwise}}
    \end{cases} + \begin{cases}
        R[[P(w)[i - 1, w[i]], \uparrow, h] &  L_{\downarrow}^{k, h}(w)[i] = L_{\downarrow}^{k, h}(w)[[P(w)[i - 1, w[i]]] + 1\\
        0 & \text{\emph{otherwise}}
    \end{cases}.
    \]
    Observing that Algorithm \ref{alg:computing_R_w} computes the above summation, we have the correctness of the algorithm. To determine the time complexity, note that for each set $i \in [n], h \in [k]$ we perform $O(\sigma)$ additions to determine the values of $R(w,k)[i, \uparrow, h]$ and $R(w,k)[i, \downarrow, h]$. As there are $n k$ total values of $i \in [n], h \in [k]$, we get the total complexity of $O(n \sigma k)$.\qed
\end{proof}


We now move to the problems of counting and enumerating rollercoasters.

\begin{lemma}
    \label{obs:uniqueness_of_maximum_rollercoasters}
    Given a word $w \in \Sigma^n$ and pair of rollercoasters $s$ and $s'$ such that $s = w[i_1] w[i_2] \dots w[i_m]$ and $s' = w[j_1] w[j_2] \dots w[j_m]$ where $m$ is the length of the longest rollercoaster that is a subsequence of $w$, either $s \neq s'$ or $(i_1, i_2, \dots, i_m) = (j_1, j_2, \dots, j_m)$.
\end{lemma}

\begin{proof}
    If $(i_1, i_2, \dots, i_m) = (j_1, j_2, \dots, j_m)$ then clearly $s = s'$. Assuming, therefore, that $(i_1, i_2, \dots, i_m) \neq (j_1, j_2, \dots, j_m)$, we have that $s = s'$ if and only if $w[i_c] = w[j_c], \forall c \in [m]$. Let $t \in [m]$ be the value such that $i_1, i_2, \dots, i_{t - 1} = j_1, j_2, \dots, j_{t - 1}$ and $i_t \neq j_t$. If $s = s'$ then $w[i_t] = w[j_t]$. If $i_t < j_t$ then $w[i_1] w[i_2] \dots w[i_t] w[j_t] w[j_{t + 1} \dots w[j_{m}]$ must be a rollercoaster of length $m + 1$, contradicting the assumption that $m$ is the length of the longest rollercoaster in $w$. Analogously, if $i_t > j_t$, $w[j_1] w[j_2] \dots w[j_t] w[i_t] w[i_{t + 1} \dots w[i_{m}]$ must be a rollercoaster. Hence the claim holds.\qed
\end{proof}

\begin{lemma}
    \label{lem:counting_maximum_rollercoasters}
    Let $w \in \Sigma^n$ be a word where the length of the longest rollercoaster in $w$ is $m$. Then, the total number of rollercoasters in $w$ of length $m$ is given by
    $$\sum\limits_{i \in [n], \xi \in \{\uparrow, \downarrow\}} R(w,k)[i, m, \xi, 0].$$
\end{lemma}

\begin{proof}
    Following Lemma \ref{obs:uniqueness_of_maximum_rollercoasters}, any rollercoaster of maximum length $m$ in $w$ must be unique. Therefore, given any pair of indices $i, i' \in [n]$, any $m$-length rollercoaster ending at $w[i]$ must be distinct from any such rollercoaster ending at $w[i']$. Hence the above statement holds.
\end{proof}

% \begin{observation}
%     \label{obs:reverse_has_the_same_number_of_rollercoasters}
%     Given a word $w$ and subsequence of $w$, $s = w[i_1] w[i_2] \dots w[i_m]$, $s$ is a rollercoaster in $w$ if and only if $w[i_m] w[i_{m - 1}] \dots w[i_1]$ is a rollercoaster. 
% \end{observation}

% \begin{observation}
%     \label{obs:using_the_roller_coaster_table_to_get_the_number_of_smaller_coasters}
%     Given a word $w$, index $i \in [n]$ such that $m$ is the length of the longest rollercoaster in $w$, the number of $m$-length rollercoasters in $w$ starting at $w[i]$ is equal to $R(w^R)[n - i, m, \uparrow, 0] + R(w^R)[n - i, m, \downarrow, 0]$.
% \end{observation}

In order to enumerate the set of rollercoasters in a given word $w$, we need one additional auxiliary structure, the \emph{next element graph} of $w$, denoted $NEG(w)$. We define $NEG(w) = (V, E)$ as a directed graph with every edge labelled with one of $\{\uparrow, \rightarrow, \downarrow\}$, where $V = v_1, v_2, \dots, v_n$, with $v_i$ used to represent $w[i]$, and an edge $(v_i, v_j)$ (starting at $v_i$, ending at $v_j$), where $i < j$, and labelled by $\xi \in \{\uparrow, \rightarrow, \downarrow \}$ if and only if:
\begin{itemize}
    \item $\xi = \uparrow$, $w[i] < w[j]$ and $\forall j' \in [i + 1, j - 1], w[i] > w[j']$ or $w[j'] > w[j]$,
    \item $\xi = \rightarrow$, $w[i] = w[j]$ and $i = P(w)[j - 1, w[j]]$, or,
    \item $\xi = \downarrow$, $w[i] > w[j]$ and $\forall j' \in [i + 1, j - 1], w[i] < w[j]$ or $w[j'] < w[j]$.
\end{itemize}

\begin{observation}
    Every maximum length rollercoaster in $w$ corresponds to a path in $NEG(w)$.
\end{observation}

\begin{lemma}
    \label{lem:constructing_NEG}
    Given a word $w \in \Sigma^n$, $NEG(w)$ can be constructed in $O(n \sigma)$ time.
\end{lemma}

\begin{proof}
    We achieve this by working backwards, adding in-edges to each vertex. We note out construction does not rely on the ordering of the vertices, and therefore it is sufficient to prove that our construction adds all in edges to the current vertex $v$. Given the vertex $v_j$, we claim that there exists some edge starting at $v_i$ and ending at $v_j$ labelled by $\uparrow$ if and only if $i \in \{P(w)[j - 1, x] \mid x \in [w[j] - 1], \forall x' \in [x + 1, w[j]], P(w)[i - 1, x'] < P(w)[i - 1, x]\}$. Observe that, by the definition of $NEG(w)$, any position $i'$ not in this set either contains a symbol greater than or equal to $w[j]$, and thus can not be used as a unique symbol in an increasing run, or is followed by some $x$ such that $w[i'] \leq x \leq w[j]$, and therefore a longer increasing run can be formed by inserting $x$ between $w[i]$ and $w[j]$. In the other direction, given any $i \in \{P(w)[j - 1, x] \mid x \in [w[j] - 1], \forall x' \in [x + 1, w[j]], P(w)[i - 1, x'] < P(w)[i - 1, x]\}$, any $i' \in [i + 1, j - 1]$ satisfies either $w[i'] < w[i]$ or $w[i'] > w[j]$, and hence the edge $(v_i, v_j)$ labelled $\uparrow$ exists in $NEG(w)$. We construct the set $\{P(w)[j - 1, x] \mid x \in [w[j] - 1], \forall x' \in [x + 1, w[j]], P(w)[i - 1, x'] < P(w)[i - 1, x]\}$ in $O(\sigma)$ time by checking each $x \in [w[j] - 1]$ in decreasing order if $P[j - 1, x] < P(w)[i - 1, x'], \forall x' \in [x + 1, w[j]]$. By storing some value $p$ corresponding to $\max_{x' \in [x + 1, w[j]]} P(w)[j - 1, x']$, initially set to $P(w)[j - 1, w[j]]$, we can determine if this holds in $O(1)$ time, updating $p$ to $\max(P(w)[j - 1, x], p)$ after checking each value of $x$, allowing the set to be constructed in $O(\sigma)$ time, and thus all in-edges ending at $v[j]$ labelled by $\uparrow$ to be determined in $O(\sigma)$ time. By analogous techniques, we can determine the set of in-edges ending at $v[j]$ labelled by $\downarrow$ in $O(\sigma)$ time. Finally, the edge labelled $\rightarrow$ can be determined from $P(w)$ in constant time, and therefore $NEG(w)$ can be constructed in $O(n \sigma)$ time.
\end{proof}

We provide pseudo code for constructing $NEG(w)$ in Algorithm \ref{alg:constructing_NEG}

\begin{algorithm}
\textbf{Input:} $w \in \Sigma^n$, $k \in \mathbb{N},$ Rllercoaster table $R(w, k)$\\
\textbf{Output:} rollercoaster table $R$ for $w$ and $k$
\begin{lstlisting}[mathescape=true]
Initialise $L_{\xi}^{k, h}(w)$, $\forall \xi \in \{\uparrow, \downarrow\}, h \in [k]$
Compute $P(w)$
Set $V = \{ v_1, v_2, \dots, v_n\}$
Set $E = \emptyset$ // We store the edges as tripples $(v_i, v_j, \xi)$, where $v_i$ is the start, $v_j$ is the end, and $\xi$ is the label.
for $i \in [2, n]$ // itteration over the vertices in the graph to add the edges. Note that $v_1$ has no incoming edges.
    $p_{\uparrow} = P[i - 1, w[i]]$ // initail bound on which $\uparrow$-labelled edges are blocked by existing edges, note that we do not need to explicitly construct the set $\{P(w)[i - 1, x] \mid x \in [w[i] - 1], \forall x' \in [x + 1, w[i]], P(w)[i - 1, x'] < P(w)[i - 1, x]\}$
    for $x \in w[i] - 1, w[i - 1] \dots, 1$ // check each value of $x$ in descending order
        if $P(w)[i - 1, x] > p_{\uparrow}$ // if $P(w)[i - 1, x]$ appears after every symbol in $w$ labelled by some $x' \in x + 1, w[i]$, then we add an edge and update $p$
            $E = E \cup \{ (v_{P(w)[i - 1, x]}, v_i, \uparrow)\}
            $p_{\uparrow} = \max(p_{\uparrow}, P(w)[i - 1, x])$
    $p_{\downarrow} = P[i - 1, w[i]]$ // We now do the same for the edges labelled $\downarrow$
    for $x \in w[i] + 1,  \sigma$
        if $P(w)[i - 1, x] > p_{\downarrow}$ // if $P(w)[i - 1, x]$ appears after every symbol in $w$ labelled by some $x' \in w[i], x - 1, w[i]$, then we add an edge and update $p_{\downarrow}$
            $E = E \cup \{ (v_{P(w)[i - 1, x]}, v_i, \downarrow)\}
            $p_{\downarrow} = \max(p_{\downarrow}, P(w)[i - 1, x])$
    $E = E \cup \{(v_{P[i - 1, w[i]]}, v_i, \rightarrow)\}$ // Finally, we add the labelled $\rightarrow$ from $v_{P(w)[i - 1, w[i]}$ to $v_i$ 
return $(V, E)$
\end{lstlisting} 
\caption{Construct$NEG$}\label{alg:constructing_NEG}
\end{algorithm}

\begin{observation}
    \label{obs:every_path_is_unique}
    Given a word $w \in \Sigma^n$, let $i_1, i_2, \dots, i_{\sigma}$ be the set of position such that $w[i_q] = q$ and $\forall i' \in [i_q - 1], w[i'] \neq q$. Every path of length $j$ in $NEG(w)$ starting at any vertex $v_{i_q}$ corresponds to a unique subsequence of $w$.
\end{observation}

\begin{proof}
    Assume, for the sake of contradiction, that there exists some pair of paths $P = v_{p_1}, v_{p_2}, \dots, v_{p_j}$, and $Q = v_{q_1}, v_{q_2}, \dots, v_{q_j}$, where $w[p_1] w[p_2] \dots w[p_j] = w[q_1] w[q_2] \dots w[q_j]$. Now, as $w[p_1] = w[q_1]$, both $P$ and $Q$ must start at vertex $v_{w[p_1]}$, so $p_1 = q_1$. Similarly, observe that if the edge $(v_{p_1}, v_{p_2})$ exits in $NEG(w)$, and $w[p_2] = w[q_2]$, then $(v_{p_1}, v_{q_2})$ exists in $NEG(w)$ if and only if $p_2 = q_2$. In general, if $p_1, p_2, \dots, p_{i - 1} = q_1, q_2, \dots, p_{i - 1}$, as $w[p_i] = w[q_i]$, we have that if the edge $(v_{p_{i - 1}}, v_{p_i})$ exists in $NEG(w)$, the edge $(v_{p_{i - 1}}, v_{q_i})$ is in $NEG(w)$ if and only if $p_i = q_i$, completing the proof.
\end{proof}

\begin{lemma}
    \label{lem:every_maximum_length_rollercoaster_is_a_path}
    Given a word $w \in \Sigma^n$ and rollercoaster $u$ such that $u$ is a subsequence in $w$, and $\vert u \vert$ is the length of the longest rollercoaster of $w$, there exists exactly $1$ path of in $NEG(w)$, $i_1, i_2, \dots, i_{\vert u \vert}$ such that $w[i_1] w[i_2] \dots w[i_{\vert u \vert}] = u$.
\end{lemma}

\begin{proof}
    Let $i_1$ be the value such that $\forall i \in [i_1 - 1], w[i] \neq u[1]$ and $u[1] = w[i_1]$, and $i_2$ be the value such that $\forall j \in [i_1 + 1, i_2 - 1]$, $u[2] \neq w[j]$. As $u$ is maximal in $w$, there must be the edge $(v_{i_1}, v_{i_2})$ in $NEG(w)$, as otherwise there exists some $i' \in [i_1 + 1, i_2 - 1]$ such that either $w[i_1] \leq w[i'] \leq w[i_2]$ or $w[i_1] \geq w[i'] \geq w[i_2]$, contradicting the assumption that $u$ is a maximum length rollercoaster in $w$. Repeating this argument for every index $i_j \in \{i_1, i_2, \dots, i_{\vert u \vert}\}$ proves the statement.
\end{proof}

In order to use $NEG(w)$, we label each vertex $v_i$ with two lists, $L_{i, \uparrow}, L_{i, \downarrow}$, of length $k$ where:
\begin{itemize}
    \item $L_{i, \uparrow}[h]$ constrains the number suffixes of rollercoasters in $w$ of maximum length containing an increasing run where $w[i]$ is the $h^{th}$ unique element in the run, and the length $m_{i,j,\uparrow}$ such that $R(w^R)[n - i, m_{i, j, \uparrow}, \uparrow, j] > 0$ and, $\forall m' \in [m_{i, j, \uparrow}, n], R(w^R)[n - i, m', \uparrow, j] = 0$,
    \item $L_{i, \downarrow}[j]$ constrains the number suffixes of rollercoasters in $w$ of maximum length containing an increasing run where $w[i]$ is the $j^{th}$ unique element in the run, and the length $m_{i,j,\downarrow}$ such that $R(w^R)[n - i, m_{i, j, \downarrow}, \downarrow, j] > 0$ and, $\forall m' \in [m_{i, j, \downarrow}, n], R(w^R)[n - i, m', \downarrow, j] = 0$.
\end{itemize}

% Using $R(w, k)$, we can determine the value of $L_{i, \xi}[h]$, for every $i \in [n], h \in [k]$ and $\xi \in \{ \uparrow, \downarrow\}$ in $O(n k)$.

We use $NEG(w)$ to enumerate the set of all maximum length rollercoasters in a recursive manner. At a high level, the idea is to work backwards, using the tables $L_{\xi}^{k, h}$ to determine which positions in $w$ correspond to the final positions in maximum length plateau $k$-rollercoasters in $w$. Once the last symbol has been determined, we use the edges in $NEG(w)$ to determine which preceding positions can be used to construct value runs ending at the appropriate position. We repeat this until we have determined the a valid rollercoaster, which we then output. By using the the rollercoaster table, we can check efficiently if a given position is valid, with $R(w, k)[i, \xi, h]$ denoting the number partial plateau $(k, h)$-rollercoaster ending at $i$, and therefore if the number of prefixes of length $L_{\xi}^{k, h}[i]$ ending at $i$.

\begin{observation}
    \label{obs:final_position}
    Given a word $w \in \Sigma^n$, integer $k$, and rollercoaster $s = w[i_1] w[i_2] \dots w[i_m]$ that is a maximum length plateau $k$-rollercoaster in $w$, $i_m = P(w)[n, w[i_m]]$.
\end{observation}

\begin{proof}
    Assume, for the sake of contradiction, that this does not hold. Then, there must be some rollercoaster $s = w[i_1] w[i_2] \dots w[i_m]$ where $i_m \notin P(w)[n]$. However, observe that $s w[P(w)[n, w[i_m]]]$ is also a plateau $k$-rollercoaster in $w$ and has longer length than $s$, contradicting the initial assumption, and hence the statement holds.
\end{proof}

\begin{theorem}
    \label{thm:enumerating_rollercoasters}
    Given a word $w \in \Sigma^n$ and integer $k \in \mathbb{N}$, where $m$ is the length of the longest plateau $k$-rollercoaster in $w$, there exists an algorithm outputting all plateau $k$-rollercoasters in $w$ of length $m$ with $O(n)$ delay after $O(n \sigma k)$ preproccesing.
\end{theorem}

\begin{proof}
    Before we begin the enumeration, as our preproccessing step, we compute the tables $L_{\xi}^{k, h}(w)$ for every $h \in [k]$, $P(w)$, the rollercoaster table $R(w, k)$ and the next element graph $NEG(w) = (V, E)$, requiring $O(n \sigma k)$ time. Further, we use $m$ to denote the length of the longest plateau $k$-rollercoaster in $w$.

    To determine the first rollercoaster, let $i_m$ be some index such that $i_m = P(w)[n, x]$, for some $x \in \Sigma$, and $L_{\xi}^{k, k}(w)[i_m] = m$, for some $\xi \in \{\uparrow, \downarrow\}$. By construction, there must exist some plateau $k$-rollercoaster ending with a $\xi$ run at $i_m$ and further, the preceding position $i_{m - 1}$ must satisfy either $(v_{i_{m - 1}}, v_{i_m}, \xi) \in E$, $L_{\xi}^{k, k}(w)[i_m] = L_{\xi}^{k, h}(w)[i_{m - 1}] + 1$, for some $h \in \{k - 1, k\}$, or $(v_{i_{m - 1}}, v_{i_m}, \rightarrow) \in E$, and $L_{\xi}^{k, k}(w)[i_m] = L_{\xi}^{k, k}(w)[i_{m - 1}] + 1$. We can determine the value of $i_{m - 1}$ by checking each incoming edge $(v_{j}, v_{i_m}, \xi)$ and the edge $(v_j, v_{i_m}, \rightarrow)$ in at most $O(\sigma)$ time. We assume, without loss of generality, that we choose the value of $i_{m - 1}$ satisfying $\forall j \in [i_{m - 1} + 1, i_m - 1]$, either $(v_{i_{m - 1}}, v_{i_m}, \xi) \notin E$, $(v_{i_{m - 1}}, v_{i_m}, \rightarrow) \notin E$, $(v_{i_{m - 1}}, v_{i_m}, \xi) \in E$ and $L_{\xi}^{k, h'}[j] + 1 < L_{\xi}^{k, k}[i_m], \forall h' \in \{k - 1, k\}$, or $(v_{i_{m - 1}}, v_{i_m}, \rightarrow) \in E$ and $L_{\xi}^{k, k}[j] + 1 < L_{\xi}^{k, k}[i_m]$.

    In general, once the value of $i_j$ has been determined, we determine the value of $i_{j - 1}$ as follows. Let us assume that $i_j$ is the $h^{th}$ unique element of a $\xi$-run. If $h \geq k$, then $i_{j - 1}$ must be some index such that $(v_{i_{j - 1}}, v_{i_{j}}, \xi) \in E$ and $L_{\xi}^{k, h'}[j - 1] + 1 = L_{\xi}^{k, k}[j]$, for some $h' \in \{\{k - 1, k\} \}$, or $(v_{i_{j - 1}}, v_{i_{j}}, \rightarrow) \in E$, and $L_{\xi}^{k, k}[j - 1] + 1 = L_{\xi}^{k, k}$. If $h \in [2, k - 1]$, then $i_{j - 1}$ must satisfy either $(v_{i_{j - 1}}, v_{i_{j}}, \xi) \in E$ and $L_{\xi}^{k, h - 1}[j - 1] + 1 = L_{\xi}^{k, h}[j]$, or $(v_{i_{j - 1}}, v_{i_{j}}, \rightarrow) \in E$, and $L_{\xi}^{k, h}[j - 1] + 1 = L_{\xi}^{k, h}$. Finally, if $h = 1$, then $i_{j - 1}$ must satisfy either $(v_{i_{j - 1}}, v_{i_{j}}, \overline{\xi}) \in E$ and $L_{\xi}^{k, h'}[j - 1] + 1 = L_{\xi}^{k, k}[j]$, for some $h' \in \{\{k - 1, k\} \}$, or $(v_{i_{j - 1}}, v_{i_{j}}, \rightarrow) \in E$, and $L_{\xi}^{k, h'}[j - 1] + 1 = L_{\xi}^{k, 1}$, for some $h' \in \{\{k - 1, k\} \}$. In all cases, we can determine this in $O(\sigma)$ time by checking each incoming edge to $v_{i_j}$ in order, terminating once a valid index has been found $i_{j - 1}$. Further, we assume that $i_{j - 1}$ is the largest index satisfying this condition and further that we check each candidate index from largest to smallest.

    To get the delay in the first output, observe that no index is checked as a candidate to be added to the rollercoaster more than once. Therefore, as there are at most $n$ possible checks, the total delay is $O(n)$.

    To determine the next rollercoaster after outputting the rollercoaster $s = w[i_1] w[i_2] \dots w[i_m]$, we require an auxiliary set of $m$ counters, $c_1, c_2, \dots, c_m$, where $c_j$ counts the number of rollercoasters that have been output so far with the suffix $w[i_j] w[i_{j + 1}] \dots w[i_{m}]$. Note that if $c_j < R(w, k)[i_j, \xi, h]$, where $w[i_j]$ is the $h^{th}$ (or at least $h^{th}$ if $h = k$) unique symbol in a $\xi$-run in $s$, then there exists some rollercoaster with the suffix $w[i_j] w[i_{j + 1}] \dots w[i_m]$ that has not been output and otherwise every rollercoaster with this suffix has been output. Now, let $j$ be the value such that $c_j < R(w, k)[i_j, \xi_j, h_j]$ and $c_{j'} = R(w, k)[i_{j'}, \xi_{j'}, h_{j'}]$, for every $j' \in [j - 1]$ where $i_{f}$ is the $h_{f}^{th}$ unique symbol in a $\xi_f$ run in $s$. We construct the new rollercoaster by first finding the new value $i_{j - 1}'$ in the same manner as for the first rollercoaster, with the additional constraint that $i_{j - 1}' < i_{j - 1}$. Once $i_{j - 1}'$ has been determined, we find the value of $i_{j'}$, for every $j' \in [j - 2]$ in the same manner as above, without any additional restriction on the maximum value. Again, by choosing the largest possible value for $i_{j'}'$ each time, we ensure that at most $O(n)$ comparisons are needed, and thus the delay between output is at most $O(n)$. Once the new set of indices has been determined, we output the new rollercoaster $s = w[i_1'] w[i_2'] \dots w[i_{j - 1}'] w[i_j] w[i_j + 1] \dots w[i_m]$, and update the value of $c_{j'}$ to $1$, if $j' < j$, or to $c_{j'} + 1$ if $j' \geq j$.
    
    To show correctness, observe that each output corresponds to a unique path in $NEG(w)$, and thus, by Observation \ref{obs:every_path_is_unique}, a unique rollercoaster. Further, as we output $R(w, k)[i_j, \xi h]$ rollercoasters with the suffix $w[i_j] w[i_{j + 1}], \dots, w[i_{m}]$, when $w[i_j]$ is the $h^{th}$ element on a $\xi$ run, we must output every possible such rollercoaster, completing the proof.
\end{proof}


==> upperbounds.tex <==
\section{Edit Distance - Upper bounds}


Here, we present two upper bounds, one for the single symbol swap, and one for the insertion operation.

\subsection{Single Symbol Swap}

\begin{definition}
	For $w \in \Sigma^*$, the word obtained via a \emph{single symbol swap operation} from position $i$ to position $j$, $i,j \in [|w|]_0$ is defined by
	\[
	\begin{cases}
		w[1..j] w[i] w[j+1..i-1] w[i+1..|w|] & \text{, if $i > j$}\\
		w[1..i-1] w[i+1..j-1] w[i] w[j..|w|] & \text{, if $i<j$}\\
		w & \text{, otherwise.}
	\end{cases}
	\]
\end{definition}

Here, we provide the following results:
\begin{itemize}
    \item Given a sequence $S$ where $\vert S \vert \geq (\ell + c)(k - 1) + 1$ containing a rollercoaster with $\ell$ $k$-runs we can construct a sequence $S'$ with $\ell + c$ $k$-runs, using at most $c(k - 1)$ single symbol swaps from $S$.
    \item Given a sequence $S$ where $\vert S \vert \geq m + c$ containing a rollercoaster $R$ of length $m$ we can construct a sequence $S'$ containing some rollercoaster $R'$ of length $m + c$ with the same number of runs as $R'$.
\end{itemize}

\paragraph*{Drap and Drop Algorithm}

We achieve our first result via an algorithm we call the ``drag and drop'' algorithm. We use the following observation as the basis for this algorithm.

\begin{observation}
    \label{obs:moving_symbols_forward}
    Given a sequence $S$ containing a rollercoaster $R$ of $2$ $k$-runs at the position $r_{1,1}, r_{1,2}, \dots, r_{1, k}$ and $r_{2, 1}, r_{2, 2}, \dots, r_{2, k}$, where $r_{1,k} = r_{2, 1}$, and some position $i$ such that $i \notin R$ and $i < r_{1, k}$. Then, there exists some sequence $S'$ formed by making a single symbol swap from $S[i]$ to $i'$ such that $S'$ contains a rollercoaster $R'$ of $2$ $k$-runs $R' = r'_{1,1}, r'_{1,2}, \dots, r'_{1, k}$ and $r'_{2, 1}, r'_{2, 2}, \dots, r'_{2, k}$, where $r'_{1,k} = r'_{2, 1}$ and $i' = r'_{x, k}$, for some $x \in [1, k]$.
\end{observation}

\begin{proof}
    Let us assume, without loss of generality, that $R$ starts with a decreasing run ($r_1$) then has an increasing run ($r_2$).
    Note that as $i \notin R$, $S[i] < S[r_{1, k}]$. Now, let $r_{2, y}$ be the position such that $S[r_{2, y}] > S[i] > S[r_{2, y + 1}]$, or $r_{2, k}$ if $S[r_{2, k}] > S[i]$. Now, observe that for any $i' \in [r_{2, y} + 1, r_{2, y + 1}]$, the sequence $S' = S[1, i - 1] S[i + 1, i'] S[i] S[i' + 1, \vert S \vert]$ contains the rollercoaster $R'$ of length $\vert R \vert + 1$.
\end{proof}

Observation \ref{obs:moving_symbols_forward} provides the basis for our first result, namely increasing the length of the longest rollercoaster.

\begin{lemma}
    Given a sequence $S$ where $R$ is the longest rollercoaster in $S$ and $\vert S \vert > \vert R \vert$, there exists some sequence $S'$ formed by making a single symbol swap from $S$ where the longest rollercoaster in $S'$ has length at least $\vert R \vert + 1$.
\end{lemma}

\begin{proof}
    We consider two cases, where $R$ contains a single run, and the general case.

    First, assume that $R$ contains only one run, and further that $R$ is increasing. Given some $i \in [1, \vert S \vert] \setminus R$, note that there must be some $r < i$ such that $S[r] > S[i]$. Let us assume that $r \in R$ is the smallest postion such that $S[r] > S[i]$, i.e. the position such that $S[r] > S[i]$ and $\forall r' \in [R], r' < r, S[r'] < S[i]$. Then, the sequence $S' = S[1, r - 1] S[i] S[r, i - 1] S[i + 1, \vert S \vert]$ contains the rollercoaster $R' = \{a \in R \mid a \leq r\} \cup \{b + 1 \mid b \in R, b > r\}$ and thus the longest rollercoaster in $S'$ is longer than the longest rollercoaster in $S$.

    Otherwise, we can apply the same technique as in Observation \ref{obs:moving_symbols_forward} to create the sequence $S'$. Note that for any $i$ where $i \in [1, \vert S \vert] \setminus R$ and $i$ is after some position $r \in R$ belonging to the final run of $R$, the same arguments can be applied to move the symbol $S[i]$ to the penultimate run, achieving the same increase.
\end{proof}

\begin{corollary}
    Given a sequence $S$ where $R$ is the longest rollercoaster in $S$ and $\vert S \vert > \vert R \vert + c$, there exists some equence $S'$ formed by $c$ single symbol swaps from $S$ where the longest rollercoaster in $S'$ has length at least $\vert R \vert + c$.
\end{corollary}

Now, we move to the problem of constructing rollercoasters containing more runs, while having the same or greater length.

\begin{lemma}
    Let $S$ be a sequence where $R$ is the rollercoaster in $S$ with the largest number of $k$-runs, and let $\ell$ be the number of runs in $R$. Then, a sequence $S'$ can be constructed containing some $k$-run rollercoaster $R'$ with $\ell + 1$ runs and length $\vert R' \vert \geq \vert R \vert$ using $\ell(k - 1)$ single swaps.
\end{lemma}

\begin{proof}
    We use the same approach as outlined in Observation \ref{obs:moving_symbols_forward}. Given $S$, we find the right-most position $i$ such that either $i \notin R$ or the run containing $i$ has at least $k + 1$ symbols and $i$ is not the last symbol in the run. Using this, we can move $S[i]$ to some position in the subsequent run. We repeat this until there are $k - 1$ symbols after the last run in $R$, all of which are either greater than the last symbol in the run, if it is a decreasing run, or less than the last symbol if it is an increasing run. We may assume that these symbols are sorted in either increasing or decreasing order as they are moved into the new positions. As there are $\ell$ runs, it is nessesary to make at most $\ell$ swaps to move some symbol after the last run in $S$. Further, as each run requires $k$ symbols, one of which is the last symbol of the previous run, it is nessesary to make at most $\ell(k - 1)$ swaps. Note that at each step the length of the longest rollercoaster decreases if and only if the swap ends with the symbol being placed after the last run, and any symbol moved to after the last run is added to the new run after the final swap. Therefore, the length of $R'$ is at least the length of $R$, completing the proof.
\end{proof}

\subsection{Insertion}

\begin{lemma}
    \label{lem:insertion_increasing_length}
    Let $S$ be a sequence where the subsequence $R$ is the longest rollercoaster in $S$. Then a sequence $S'$ can be formed by insterting some symbol into $S$ such that the longest rollercoaster $R'$ in $S'$ has length $\vert R' \vert > \vert R \vert$.
\end{lemma}

\begin{proof}
    Triv.
\end{proof}

\begin{corollary}
    \label{col:insertion_works_with_any_symbol}
    Let $S$ be a sequence where the subsequence $R$ is the longest rollercoaster in $S$. Then a sequence $S'$ can be formed by insterting some given symbol into $S$ such that the longest rollercoaster $R'$ in $S'$ has length $\vert R' \vert > \vert R \vert$.
\end{corollary}

\begin{proof}
    Same as above but now the symbol we are inserting is fixed.
\end{proof}

\begin{lemma}
    \label{lem:insertion_increasing_runs}
    Let $S$ be a sequence where the subsequence $R$ is the longest $k$-run rollercoaster in $S$. Then a sequence $S'$ can be formed by insterting $k - 1$ symbols into $S$ such that the longest rollercoaster $R'$ in $S'$ has at least 1 more $k$-run than $S$.
\end{lemma}

\begin{proof}
    Just add them to the end
\end{proof}

\subsection{Deletion}

In this section we give for a sequence $S$ and its longest rollercoaster the maximal number of deletions we can perform to still obtain a rollercoaster with the same amount of runs.

\begin{observation}
	Let $S$ be a sequence where the subsequence $R$ is the longest $k$-rollercoaster in $S$. Then a sequence $S'$ can be formed by deleting at least $|S| -|R|$ symbols in $S$ such that $S'$ is a $k$-rollercoaster and constis of an equal number of runs as $R$.
\end{observation}
\begin{proof}
	First notice that deleting every letter that does not belong to $R$ can be done immediately. 
	Furthermore, we can concurrently save the length of each run during this first pass through $S$. Let $\ell$ be the number of runs in $R$ and $l_1, \ldots, l_\ell \in \N \geq k$ the runs' lengths. Within a second pass through $R$ we can now delete letters in the following positions to obtain the shortest sequence $S'$ is a $k$-rollercoaster and constis of an equal number of runs as $R$:
	\begin{align*}
		r_i[j] \quad \text{, if $l_{i}>k$ and $j \in [2,l_i -1]$}.
	\end{align*}
	Note that a deletion of the end or beginning of a run would immediately decrease the length of two runs, i.e., the resulting rollercoaster would be of longer length.
\end{proof}

\section{Substitution}

\begin{lemma}
	Given a sequence $S$ where $R$ is the longest rollercoaster in $S$ and $|S| > |R|$, then there exists some sequence $S'$ formed by $|S| - |R|$ substitutions from $S$ where the longest rollercoaster in $S'$ has length at least $|R| + (|S| -|R|)$.
\end{lemma}
\begin{proof}
	Since rollercoasters are defined over real numbers, we can use the property that between every two numbers there exists a number that lays between them. Thus, every letter at a position that is not contained in a rollercoaster can be substituted by a letter that matches the surrounding increasing or decreasing run.
\end{proof}

\todoah{the only idea I have for an additional run by now is to rename in a way that all letters that are not used in $S$ are transferred either to the front or back}

\section{Ideas gathered in the Meetings}

\begin{itemize}
	\item fix minima and maxima $\to$ how many operations from the edit distance are needed?
	\item maximise the number of runs
	\item insert allowed vs. insert not allowed (only permutation)
	\item no drag and drop allowed, only transpositions (pairwise swaps) $\to$ differentiate between neighboured positions and arbitrary positions
	\item How many deletions can be made to still obtain a rollercoaster with the same amount of min and max?
	\item new OCR operation $\to$ merge and split: replace a single character with couple of characters
	\item rollercoasters for conjugates/cyclic words
	\item rollercoasters in Lyndon words
\end{itemize}
	
\section{Meeting 8th May}
	
\begin{itemize}
	\item finite alphabet
	\item how to handle plateaux?
	\item only allow plateaux at min and max OR allow plateaux anywhere (also in inc/dec part)
	\item searching the longest such rollercoaster
	\item specify explicit runs or properties in the rollercoaster
	\item counting and ranking
	\item enumeration (positionwise order)
	\item[TODO:] Introduction and Prelims $\to$ introducing rollercoasters with plateaux?
	\item initially alphabet $[n]$ then $\N$ $\to$ adapt Florins Rollercoaster Algorithm to plateaux and different alphabets
	\item counterexample for Florins algorithm? or extend it?
	\item think of nice datastructure
	\item use dynamic programming for enumeration later?
	\item SELL IT AS A REACHABILITY PROBLEM
\end{itemize}
	

